Completely random measures for modeling power laws in sparse graphs

Network data appear in a number of applications, such as online social networks and biological networks, and there is growing interest in both developing models for networks as well as studying the properties of such data. Since individual network datasets continue to grow in size, it is necessary to develop models that accurately represent the real-life scaling properties of networks. One behavior of interest is having a power law in the degree distribution. However, other types of power laws that have been observed empirically and considered for applications such as clustering and feature allocation models have not been studied as frequently in models for graph data. In this paper, we enumerate desirable asymptotic behavior that may be of interest for modeling graph data, including sparsity and several types of power laws. We outline a general framework for graph generative models using completely random measures; by contrast to the pioneering work of Caron and Fox (2015), we consider instantiating more of the existing atoms of the random measure as the dataset size increases rather than adding new atoms to the measure. We see that these two models can be complementary; they respectively yield interpretations as (1) time passing among existing members of a network and (2) new individuals joining a network. We detail a particular instance of this framework and show simulated results that suggest this model exhibits some desirable asymptotic power-law behavior.

==> background.tex <==
\section{Background} % and motivation}
\label{sec-background}

In this section, we first review the traditional notion of
\emph{vertex-exchangeability} for
graphs and then discuss a different notion of \emph{edge-exchangeability} for graphs.
We then review completely random measures.

\subsection{Exchangeability for graphs}

Exchangeability for graphs has traditionally been as the distribution of the
graph being invariant under permuations of the vertices.
In this sense,
a random graph $G$ %on $\Nats$
is \defn{vertex-exchangeable} if its joint distribution is invariant under all
permutations $\pi$ of the vertices:
\begin{align}
    (G_{ij})_{i,j\in\mathbb{N}} \eqdist (G_{\pi(i)\pi(j)})_{i,j\in\mathbb{N}}.
\end{align}

In edge-exchangeability (\TBD{cite}), we instead consider permutations of the
edges.
A random graph $G$ %on $\Nats$
is \defn{edge-exchangeable} if its joint distribution is invariant under all
permutations $\pi$ of the edges:
\TBD{what is the correct way of writing this?}

\TBD{Alternatively, we can view this as (give example from the other paper).
we can consider a graph as an unordered set of tuples, which represent the edges of the
graph. E.g., $E = \{\{2,3\},\{1,4\},\{3,6\}, \{6,6\},\{3,6\}\}$. In this case, we can obtain the (active) vertex set by
representing all the unique elements of $E$: $V = \bigcup_{e \in E} e$. In the previous example, $V = \{1,2,3,4,6\}$. It is not important that ``$5$'' does not appear in $V$ since the elements of $V$ are treated as arbitrary labels.
}
\TBD{make connection to feature allocation, paintboxes etc}



\subsection{Completely random measures}

A \defn{completely random measure}
$W$ on $(\Psi, \mathcal{S})$ is a random measure
such that for any finite, disjoint measurable sets
$A_1,\ldots,A_n \in \mathcal{S}$, the random variables $W(A_1),\ldots,W(A_n)$
are (pairwise) independent.
%
\citet{MR0210185} showed the completely random measures are characterized by
(1) a deterministic component, (2) a fixed atomic component, and (3) a Poisson
point process rate measure, which is known as the \emph{ordinary component} (and
also called the L\'evy measure).

Completely random measures can be constructed from a Poisson point process as
follows: draw a realization $\Pi = \{(\psi_i, U_i)\}$
from a Poisson process on $\Psi\times\Reals$ with
rate measure $\nu(d\psi, du)$ (the ordinary component).

Examples of CRMs include the beta process, the gamma process, and the Poisson
process;
see \citet[\S2]{DBLP:journals/pami/BroderickMPJ15} for more details.





